Large Synoptic Survey Telescope: Dark Energy Science Collaboration

This white paper describes the LSST Dark Energy Science Collaboration (DESC), whose goal is the study of dark energy and related topics in fundamental physics with data from the Large Synoptic Survey Telescope (LSST). It provides an overview of dark energy science and describes the current and anticipated state of the field. It makes the case for the DESC by laying out a robust analytical framework for dark energy science that has been defined by its members and the comprehensive three-year work plan they have developed for implementing that framework. The analysis working groups cover five key probes of dark energy: weak lensing, large scale structure, galaxy clusters, Type Ia supernovae, and strong lensing. The computing working groups span cosmological simulations, galaxy catalogs, photon simulations and a systematic software and computational framework for LSST dark energy data analysis. The technical working groups make the connection between dark energy science and the LSST system. The working groups have close linkages, especially through the use of the photon simulations to study the impact of instrument design and survey strategy on analysis methodology and cosmological parameter estimation. The white paper describes several high priority tasks identified by each of the 16 working groups. Over the next three years these tasks will help prepare for LSST analysis, make synergistic connections with ongoing cosmological surveys and provide the dark energy community with state of the art analysis tools. Members of the community are invited to join the LSST DESC, according to the membership policies described in the white paper. Applications to sign up for associate membership may be made by submitting the Web form at http://www.slac.stanford.edu/exp/lsst/desc/signup.html with a short statement of the work they wish to pursue that is relevant to the LSST DESC.

==> analysis/clusters/challenges.tex.tex <==
\section{Challenges and Urgent Needs}

\subsection{Major challenges} 


The major, recognized challenges to obtaining robust dark energy
constraints using galaxy clusters observed with LSST can be summarized
as follows.

A first challenge is the accurate theoretical prediction of the
distribution and clustering of galaxy clusters as a function of mass
and redshift. In particular, robust predictions for the mass and bias
functions will be required, spanning the full suite of cosmological
models and mass and redshift ranges of interest.  These predictions
should be formed in a way that facilitates fast model comparisons (see
below), for example by utilizing `universal' forms for mass and bias
functions where possible. Particularly important and challenging will
be understanding the impact of baryonic physics on these
predictions. This task will require cosmological simulations and,
likely, a significant laboratory effort, building on the
infrastructure developed for Stage III projects such as DES.

A second major challenge involves developing optimized ways to find
clusters and form catalogs, both using LSST data alone and combination
with auxiliary data. (As discussed in the analysis section, the combination of
optical and X-ray data has been shown to provide better performance
for cluster finding than optical data alone; e.g. Rykoff et
al. 2011). The challenge will be to develop algorithms that generate
cluster catalogs with maximum purity (i.e.  no false clusters) and
completeness (i.e. no clusters missing). Equally important, however,
will be the ability to quantify and model residual incompleteness and
impurity precisely, so as to be able to marginalize over these fully
in the cosmological analysis. 
This task will rely heavily upon simulated galaxy catalogues and images that accurately represent the galaxy properties of real clusters, which is a topic of intensive investigation by the DESC simulations working group.
This task will also require extensive
cosmological simulations and, likely, a significant lab effort,
building on tools set up for Stage III projects.

While theory can predict the distribution of mass quite robustly as a
function of cosmological parameters, surveys are based on {\it
observables} - measured quantities that relate to mass with complex
scaling and scatter. For LSST cluster cosmology, the primary survey
observables (in addition to photo-$z$s) will relate to optical richness,
likely augmented by X-ray and mm-wave (SZ) information. The single
most pressing challenge for cluster cosmology is to understand the
statistical relationships between galaxy cluster observables and
mass. There are two main aspects to this work: 1) understanding the
form, scatter and evolution of the {\it scaling relations} linking key
observables and mass; and 2) obtaining robust absolute mass
calibrations for these relations.

For the first aspect, nature fortunately provides several observable
quantities that are straightforward to measure and which correlate
tightly with mass, exhibiting minimal scatter across the mass and
redshift range of interest. These {\it low-scatter mass proxies}
provide a critical intermediate step, allowing one to first
statistically link survey observables to these mass proxies, and then
the mass proxies to mass. Studies have shown
(\citep[e.g.][]{Mantz0909.3098,Wu10}) that the addition of robust,
low-scatter mass proxy measurements for even a small fraction (a few percent) of the clusters in a survey can boost the overall cosmological
constraining power by factors of a few or more.  Major challenges for
this work include identifying the optimal combinations of mass proxies
for LSST cluster science; how to distribute targeted follow-up
measurements of mass proxies across the survey flux/redshift range;
where thresholding and binning can be effectively applied; quantifying
and modeling the impacts of systematic uncertainties; and actively
gathering the mass proxy data. This last challenge will involve
collaborations with other agencies, as many of the best mass proxies are provided by X-ray observations.

Equally important is the absolute mass calibration of these
mass-observable scaling relations - currently the dominant systematic
uncertainty for cluster cosmology.  Here weak lensing measurements
will play the driving role. The effects of triaxiality, projected structures along the line of sight, and the finite number of background galaxies with measurable shapes together introduce a scatter of $\geq 20$\% into shear measurements for {\it individual} clusters \citep{Becker10}, making weak 
lensing mass a relatively poor mass proxy.
Critically, for {\it ensembles} of clusters, nearly unbiased results
on the mean mass can be obtained \citep{Corless09,Becker10}. This
requires the use of selected radial fitting ranges and
detailed photometric redshift information for the lensed galaxy
population (Applegate et al. 2012). In this context, some of the most
important and pressing challenges for LSST cluster science are the
development of optimized weak lensing methods for cluster mass
calibration, identifying the optimal radial ranges over which
measurements should be made; the set of shear profile models that
should be fitted; how best to bin, stack and threshold data; whether
higher order lensing effects can be effectively utilized; and how best
to quantify and model the impacts of systematic uncertainties,
allowing these to be marginalized over in the cosmological
analysis. Correlation between lensing measurements and observables that are used to ``stack'' clusters must be quantified and accounted for to avoid bias to the dark energy constraints (\citep{Rykoff08,NohCohn12}).
Here cosmological and ImSim simulations will play an
essential role.

Galaxy clusters are crowded environments hosting the highest densities
of galaxies in the Universe. A challenge for cluster cosmology will be
mitigating and modeling the systematic effects associated with source
confusion, and contamination of lensing and other signatures by the
cluster member galaxy population.  Being the most massive objects in
the Universe, clusters also exhibit the strongest lensing
signals. Understanding how to utilize higher order lensing effects, as
well as tomographic lensing signals in both the weak and strong
lensing regimes, represent additional challenges for the DESC clusters
team.

As with other LSST probes, certain aspects of cluster cosmology, and
particularly those related to lensing measurements, are sensitive to
photo-$z$ systematics. An important and pressing challenge is to 
quantify the impact of these uncertainties on cluster mass calibration, as a function of cluster mass and redshift.  These studies should explore techniques that minimize the need for exhaustive spectroscopic follow-up.  Current studies by DESC members that utilize the full photometric redshift information for the lensed galaxies in cluster fields provide some promis in this regard (Applegate et al. 2012).
Conversely,
areas where the unique environment of clusters introduces additional demands for
external calibration data should be identified urgently.

Encompassing the above is the overarching challenge of developing a
self-consistent statistical framework to model the distribution and
properties of clusters, including the mass-observable scaling
relations, accounting for surveys biases and covariances, and
marginalizing fully over systematic uncertainties. Members of the DESC
Clusters team have been at the forefront of this work in current
cluster cosmology.  Required extensions include the incorporation of
clustering into the analysis framework, along with the related
nuisance parameters.  These issues will be addressed to some extent by Stage III
projects, but LSST has substantially higher accuracy requirements, so parallel efforts within the DESC are almost certainly desirable.  End-to-end testing from cosmological simulations to
cosmological constraints will be required for this effor.

Using this modeling infrastructure, a final major challenge is
understanding the computing needs for cluster cosmology.  Currently,
using X-ray cluster catalogs with $\approx 250$ clusters and 100
multiwavelength follow-up observations, CPU farms with 500 cores
require of order a week of run time for a complete cosmological
analysis that addresses multiple questions. Scaling simplistically
(linearly) with the number of clusters, and expecting LSST cluster
catalogs to contain hundreds of thousands of clusters, one can
envisage significant computing challenges. Understanding the computing
needs and identifying optimized ways in which to speed up the analysis
while maintaining precision and accuracy, with e.g. improved
algorithms and the judicious use of binning, are important challenges
for lab based groups.  Cluster cosmology also requires significant input from cosmological simulations, which are essential to extracting precise predictions from cosmological models, to understanding the interplay between systematic sources of error, and to testing the data processing and cosmological analysis pipeline in general.  These require substantial computing resources, and significant work will be required in conjunction with the simulations working group to identify these resources.

\subsection{Urgent Priorities}

Among the most pressing challenges described above are those related
to the absolute calibration of mass-observable scaling relations using
weak lensing methods. The results from the aforementioned studies of,
e.g. the optimal radial ranges over which measurements should be made;
the set of profile models that should be fitted to clusters; how to
bin, stack and threshold data; whether higher order lensing effects
can be effectively utilized; and how to model systematic
uncertainties, will impact significantly on the long term strategy for
cluster science with LSST and may influence the development of core
LSST software.

A related urgent issue is to evaluate the performance of current LSST
deblending algorithm in crowded cluster environments, and how
this performance impacts on the mass calibration described above.  In
particular, we need to evaluate how limitations in the deblending algorithm impact
on the cosmological constraints from clusters; the degree to which these limitations can be modeled; and the requirements for improvements in the algorithm.  Here and elsewhere, the analysis will involve data from sources such as Subaru and HST, as well as ray-tracing simulations (DES data are not well-matched to this problem because of their depth and image quality).
The work will link the development of the deblending algorithm (carried out by the LSST Data Management Group) to requirements determined by its effect on cosmological constraints.
  

Equally important is a detailed, quantitative understanding of the impact of photometric redshift uncertainties on cluster science and on cluster mass calibration in particular.  Linking to this, the development of techniques that minimize the requirements for spectroscopic follow-up may have cross-cutting benefits and expedite the progress of cluster cosmology with respect to other dark energy probes. Conversely, areas where the environments of clusters place additional demands on external calibration data should be
identified urgently, allowing preparations for the gathering of these data to be made. 

The final pressing challenge (which will likely require the efforts of
the larger lab based groups) is the development of a self-consistent
statistical framework to model the observed distribution and
properties of galaxy clusters and exploit fully the cosmological
information contained within these data. This framework should enable
reliable estimates of the computing needs for LSST cluster cosmology
(which may be substantial) and robust predictions of the eventual
cosmological constraints from galaxy clusters. Efforts by the DESC in
this regard, utilizing the expertise within the collaboration, are
also very likely to be of benefit to Stage III projects.

For other challenges, we expect that significant near-term progress
will arise naturally from Stage III experiments like DES, for example
in the theoretical prediction of the distribution and clustering of
galaxy clusters across a wide range of interesting dark energy models;
and in developing methods for cluster finding and the construction of
optimized cluster catalogs. For these topics, the DESC clusters group
will stay appraised of these efforts and aim to recognize if and when
the need for DESC involvement becomes pressing.


==> authorlist_BAK.tex <==

Abate, Alexandra$^{31}$, Aldering, Greg$^{17, 32}$, Allen, Steven W.$^{28, 29}$, Ansari, Reza$^{13}$, Antilogus, Pierre$^{15}$, Applegate, Douglas$^{28}$, Astier, Pierre$^{15}$, Aubourg, Eric$^{1}$, Bahcall, Neta A.$^{25}$, Bard, Deborah$^{28}$, Barkhouse, Wayne A.$^{40}$, Bartlett, James G.$^{1, 24}$, Bean, Rachel$^{8}$, Becker, Andrew$^{45}$, Beckmann, Volcker$^{1}$, Biswas, Rahul$^{2}$, Blanc, Guillaume$^{1}$, Bongard, Sebastien$^{15}$, Bosch, James$^{25}$, Bradac, Marusa$^{33}$, Bradshaw, Andrew$^{33}$, Brunner, Robert J.$^{39}$, Burchat, Patricia R.$^{29}$, Burke, David L.$^{28}$, Cahn, Robert$^{17}$, Campagne, Jean-Eric$^{13}$, Chang, Chihway$^{28, 29}$, Cheu, Elliott C.$^{31}$, Chiang, James$^{28}$, Cinabro, David$^{46}$, Claver, Chuck$^{19, 21}$, Clowe, Douglas$^{22}$, Cohn, Joanne D$^{17, 32}$, Connolly, Andrew$^{45}$, Cooray, Asantha$^{34}$, Croft, Rupert A.C.$^{7}$, Cui, Wei$^{26}$, Cunha, Carlos$^{29}$, Dell'Antonio, Ian P.$^{4}$, Digel, Seth W.$^{28}$, Di Matteo, Tiziana$^{7}$, Dodelson, Scott$^{9, 37}$, Doré, Olivier$^{5, 11}$, Dubois, Richard$^{28}$, Dubois-Felsmann, Gregory P.$^{28}$, Ealet, Anne$^{6}$, Escoffier, Stephanie$^{6}$, Fassnacht, Chris$^{33}$, Finley, David A.$^{9}$, Fouchez, Dominique$^{6}$, Frieman, Joshua A.$^{9, 37}$, Ganga, Ken$^{1}$, Gangler, Emmanuel$^{14}$, Garzoglio, Gabriele$^{9}$, Gawiser, Eric$^{27}$, Gilman, Fred$^{7}$, Gilmore, Kirk$^{28}$, Gladney, Larry$^{43}$, Glanzman, Thomas$^{28}$, Gottschalk, Erik E.$^{9}$, Gnedin, Nickolay Y.$^{9, 37}$, Gris, Philippe$^{14}$, Guy, Julien$^{15}$, Habib, Salman$^{2}$, Heitmann, Katrin$^{2}$, Hilbert, Stefan$^{28, 29}$, Ho, Shirley$^{7}$, Hogan, Craig$^{9, 37}$, Honscheid, Klaus$^{23}$, Huard, Zachary$^{38}$, Huff, Eric M.$^{23}$, Ivezi\'{c}, \v{Z}eljko$^{45}$, Jain, Bhuvnesh$^{43}$, Jarvis, Mike$^{43}$, Jee, M. James$^{33}$, Jeltema, Tesla$^{36}$, Jha, Saurabh W.$^{27}$, Johns, Kenneth A.$^{31}$, Johnson, Anthony S.$^{28}$, Johnson, Robert P.$^{36}$, Kahn, Steven M.$^{28, 29}$, Kent, Stephen$^{9, 37}$, Kessler, Richard$^{37}$, Kiessling, Alina$^{11}$, Kim, Alex G.$^{17}$, Kirkby, David$^{34}$, Kirshner, Robert P.$^{10}$, Kovacs, Eve V.$^{2}$, Knox, Lloyd$^{33}$, Kuhlmann, Steve$^{2}$, Levi, Michael$^{17}$, Li, Guoliang$^{26}$, Lin, Huan$^{9}$, Lupton, Robert$^{25}$, Ma, Zhaoming$^{39}$, Macintosh, Bruce$^{18}$, Mandelbaum, Rachel$^{7}$, Mantz, Adam$^{37}$, Marshall, Philip. J$^{42}$, Marshall, Stuart$^{28}$, May, Morgan$^{3}$, McDonald, Patrick$^{17}$, Meadows, Brian$^{38}$, Melchior, Peter M.$^{23}$, M\'enard, Brice$^{12}$, Moniez, Marc$^{13}$, Morandi, Andrea$^{26}$, Morris, R. Glenn$^{28}$, Newman, Jeffrey A.$^{44}$, Neyrinck, Mark C.$^{12}$, Nugent, Peter$^{17, 32}$, O'Connor, Paul$^{3}$, Olivier, Scot S.$^{18}$, Padmanabhan, Nikhil$^{47}$, Pain, Reynald$^{15}$, Peng, En-Hsin$^{26}$, Perdereau, Olivier$^{13}$, Perlmutter, Saul$^{17, 32}$, Peterson, John R$^{26}$, Petrosian, Vahe'$^{29}$, Plaszczynski, Stephane$^{13}$, Pope, Adrian C.$^{2}$, Raccanelli, Alvise$^{5, 11}$, Rasmussen, Andrew$^{28}$, Reil, Kevin$^{28}$, Rhodes, Jason$^{5, 11}$, Ricker, Paul M.$^{39}$, Ricol, Jean-Stephane$^{16}$, Roe, Natalie$^{17}$, Roodman, Aaron$^{28}$, Rosenberg, Leslie$^{45}$, Roucelle, Cecile$^{1, 24}$, Russo, Stefano$^{15}$, Sako, Masao$^{43}$, Schindler, Rafe H.$^{28}$, Schmidt, Samuel J.$^{33}$, Schneider, Michael D.$^{18, 33}$, Sehgal, Neelima$^{30}$, Seljak, Uros$^{17, 32}$, Sembroski, Glenn$^{26}$, Seo, Hee-Jong$^{17, 32}$, Shipsey, Ian$^{26}$, Spergel, David$^{25}$, Soares-Santos, Marcelle$^{9}$, Spinka, Harold$^{2}$, Strauss, Michael A.$^{25}$, Stubbs, Christopher W.$^{10}$, Tao, Charling$^{6}$, Thaler, Jon J$^{39}$, Thomas, Rollin C.$^{17}$, Thorman, Paul A.$^{33}$, Tilquin, Andre$^{6}$, Trac, Hy$^{7}$, Treu, Tommaso$^{35}$, Tristram, Matthieu$^{13}$, Tyson, J. Anthony$^{33}$, von der Linden, Anja$^{29}$, Wandelt, Benjamin D.$^{39}$, Wang, Yun$^{41}$, Wechsler, Risa H.$^{28, 29}$, White, Martin$^{17, 32}$, Wittman, David$^{33}$, Wood-Vasey, W. Michael$^{44}$, Xin, Bo$^{26}$, Yoachim, Peter$^{45}$, Zentner, Andrew R.$^{44}$, Zhan, Hu$^{20}$ 

\vspace*{5mm}

\begin{table}[htdp]
\centering
{\renewcommand{\arraystretch}{0.8}
\begin{tabular}{p{10cm}p{10cm}}
$^{1}$Astroparticule et Cosmologie, IN2P3, Paris, France & $^{25}$Princeton University \\
$^{2}$Argonne National Laboratory & $^{26}$Purdue University \\
$^{3}$Brookhaven National Laboratory & $^{27}$Rutgers University \\
$^{4}$Brown University & $^{28}$SLAC National Accelerator Laboratory \\
$^{5}$California Institute of Technology & $^{29}$Stanford University \\
$^{6}$Centre Physique des Particules de Marseille, IN2P3, Marseille, France & $^{30}$Stony Brook University \\
$^{7}$Carnegie Mellon University & $^{31}$University of Arizona \\
$^{8}$Cornell University & $^{32}$University of California, Berkeley \\
$^{9}$Fermi National Accelerator Laboratory & $^{33}$University of California, Davis \\
$^{10}$Harvard University & $^{34}$University of California, Irvine \\
$^{11}$Jet Propulsion Laboratory & $^{35}$University of California, Santa Barbara \\
$^{12}$Johns Hopkins University & $^{36}$University of California, Santa Cruz \\
$^{13}$Laboratoire de l'Acc\'{e}l\'{e}rateur Lin\'{e}aire, IN2P3, Orsay, France & $^{37}$University of Chicago \\
$^{14}$Laboratoire de Physique Corpusculaire, IN2P3, Clermont-Ferrand, France & $^{38}$University of Cincinnati \\
$^{15}$Laboratoire de Physique Nucl\'{e}aire et de Hautes Energies, IN2P3, Paris, France & $^{39}$University of Illinois \\
$^{16}$Laboratoire de Physique Subatomique et de Cosmologies, IN2P3, Grenoble, France & $^{40}$University of North Dakota \\
$^{17}$Lawrence Berkeley National Laboratory & $^{41}$University of Oklahoma \\
$^{18}$Lawrence Livermore National Laboratory & $^{42}$University of Oxford \\
$^{19}$LSST Corporation & $^{43}$University of Pennsylvania \\
$^{20}$National Optical Astronomy Observatories of China & $^{44}$University of Pittsburgh \\
$^{21}$National Optical Astronomy Observatory &  $^{45}$University of Washington \\
$^{22}$Ohio University & $^{46}$Wayne State University \\
$^{23}$Ohio State University &$^{47}$Yale University \\
$^{24}$Paris Diderot University & \\
\end{tabular}
}
\end{table}


==> matrix/matrix.tex <==

\chapter[Cross-matrix by institution and task element]{Cross-matrix by institution and task element (Kahn, Jain Ð Large foldout)}
%


==> otherdata/otherdata.tex <==

\chapter[Corollary data sets]{Corollary data sets }
%

%
\section[Existing optical imaging datasets]{What existing imaging datasets are available, and how are they useful. (Tyson, Juric Ð 1 page)}


\section[Upcoming optical imaging datasets]{What upcoming datasets are available, how will we get access to them, and how will they be useful. (Jain, Kahn Ð 2 pages)}


\section[Multiwavelength imaging and spectroscopy]{Existing datasets in other wavebands, spectroscopy, etc.   (Newman, Allen Ð 2 pages)}



